Computing Floating-Point Errors by Injecting Perturbations

Floating-point programs form the foundation of modern science and engineering, providing the essential computational framework for a wide range of applications, such as safety-critical systems, aerospace engineering, and financial analysis. Floating-point errors can lead to severe consequences. Although floating-point errors widely exist, only a subset of inputs may trigger significant errors in floating-point programs. Therefore, it is crucial to determine whether a given input could produce such errors. Researchers tend to take the results of high-precision floating-point programs as oracles for detecting floating-point errors, which introduces two main limitations: (1) difficulty of implementation and (2) prolonged execution time. The two recent tools, ATOMU and FPCC, can partially address these issues. However, ATOMU suffers from false positives; while FPCC, though eliminating false positives, operates at a considerably slower speed. To address these two challenges, we propose a novel approach named PI-detector to computing floating-point errors effectively and efficiently. Our approach is based on the observation that floating-point errors stem from large condition numbers in atomic operations (such as addition and subtraction), which then propagate and accumulate. PI-detector injects small perturbations into the operands of individual atomic operations within the program and compares the outcomes of the original program with the perturbed version to compute floating-point errors. We evaluate PI-detector with datasets from ATOMU and HSED, as well as a complex linear system-solving program. Experimental results demonstrate that PI-detector can perform efficient and accurate floating-point error computation.

==> discussion.tex <==
\section{Discussion}
\label{discussion}
In this section, we discuss the implementation of perturbations and numerical error detection and practical utility. 

\textbf{Implementation of perturbations.} In our experiments, one ULP subtraction serves as the primary perturbation, except one specific case. For the ATOMU\_11 and ATOMU\_17 in Table~\ref{error_and_correlation}, DELA could not detect the significant errors if we just subtract one ULP for all the results of atomic operations. This issue is due to the perturbation offset. Ideally, if the catastrophic cancellation is the root cause of significant errors and we subtract one ULP from one of the operands which is the result of another atomic operation, the original operation \(x-y\) transforms into \(x-(y-ULP)\). Consequently, the atomic operation would lead to large difference between the two results because of the huge condition number and the perturbation. However, if \(x\) is also reduced by one ULP, both results align, and the error is effectively masked. To address this, we apply a cyclic approach by subtracting and adding one, two, and three ULPs in succession.



\textbf{Numerical Error detection and practical utility.} One of the main motivations behind DELA’s design is to address the limitations of existing high-precision error detection methods. High-precision programs often require considerable execution time, rendering them impractical for larger-scale applications or real-time systems. DELA overcomes this by introducing perturbations directly at the atomic operation level, thereby emulating rounding errors without the computational cost of full high-precision computations. Our evaluation demonstrates the effectiveness of perturbation-based techniques in identifying numerical errors induced by large atomic condition numbers. This also provides a practical guideline for developers and researchers aiming to identify critical error-prone areas in their numerical programs. 

%\textbf{Limitations and future directions.} Despite its strengths, DELA has some limitations that suggest future research. For example, in cases where atomic condition numbers are not solely responsible for large errors, e.g.,  interactions with compiler optimizations or unexpected operand values. 
% Moreover, although DELA captures a wide range of significant errors, 
%Future research can develop adaptive perturbation strategies that can automatically adjust the magnitude and frequency of perturbations based on the specific characteristics of the program and the input data. 

\begin{wrapfigure}{l}{0.5\textwidth}
    \centering
    \includegraphics[width=0.48\textwidth]{./figure/gsl_linalg_LU_decomp.pdf}
    \caption{An example of big condition number in the 3,000-dimensional linear system-solving program.}
    \label{gsl_linalg_LU_decomp}
\end{wrapfigure}
